Exploring scalable medical image encoders beyond text supervision

Language-supervised pre-training has proven to be a valuable method for extracting semantically meaningful features from images, serving as a foundational element in multimodal systems within the computer vision and medical imaging domains. However, the computed features are limited by the information contained in the text, which is particularly problematic in medical imaging, where the findings described by radiologists focus on specific observations. This challenge is compounded by the scarcity of paired imaging-text data due to concerns over leakage of personal health information. In this work, we fundamentally challenge the prevailing reliance on language supervision for learning general-purpose biomedical imaging encoders. We introduce RAD-DINO, a biomedical image encoder pre-trained solely on unimodal biomedical imaging data that obtains similar or greater performance than state-of-the-art biomedical language-supervised models on a diverse range of benchmarks. Specifically, the quality of learned representations is evaluated on standard imaging tasks (classification and semantic segmentation), and a vision-language alignment task (text report generation from images). To further demonstrate the drawback of language supervision, we show that features from RAD-DINO correlate with other medical records (e.g., sex or age) better than language-supervised models, which are generally not mentioned in radiology reports. Finally, we conduct a series of ablations determining the factors in RAD-DINO's performance; notably, we observe that RAD-DINO's downstream performance scales well with the quantity and diversity of training data, demonstrating that image-only supervision is a scalable approach for training a foundational biomedical image encoder. Model weights of RAD-DINO trained on publicly available datasets are available at https://huggingface.co/microsoft/rad-dino.

==> bibliography.tex <==
\begin{thebibliography}{127}
        \providecommand{\natexlab}[1]{#1}
        \providecommand{\url}[1]{\texttt{#1}}
        \expandafter\ifx\csname urlstyle\endcsname\relax
          \providecommand{\doi}[1]{doi: #1}\else
          \providecommand{\doi}{doi: \begingroup \urlstyle{rm}\Url}\fi
        
        \bibitem[Desai and Johnson(2021)]{desai2021virtex}
        Karan Desai and Justin Johnson.
        \newblock Virtex: Learning visual representations from textual annotations.
        \newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 11162--11173, 2021.
        
        \bibitem[Radford et~al.(2021)Radford, Kim, Hallacy, Ramesh, Goh, Agarwal, Sastry, Askell, Mishkin, Clark, et~al.]{radford2021learning}
        Alec Radford, Jong~Wook Kim, Chris Hallacy, Aditya Ramesh, Gabriel Goh, Sandhini Agarwal, Girish Sastry, Amanda Askell, Pamela Mishkin, Jack Clark, et~al.
        \newblock Learning transferable visual models from natural language supervision.
        \newblock In \emph{International conference on machine learning}, pages 8748--8763. PMLR, 2021.
        
        \bibitem[Yu et~al.(2022{\natexlab{a}})Yu, Wang, Vasudevan, Yeung, Seyedhosseini, and Wu]{Yu2022CoCaCC}
        Jiahui Yu, Zirui Wang, Vijay Vasudevan, Legg Yeung, Mojtaba Seyedhosseini, and Yonghui Wu.
        \newblock Coca: Contrastive captioners are image-text foundation models.
        \newblock \emph{Trans. Mach. Learn. Res.}, 2022, 2022{\natexlab{a}}.
        \newblock URL \url{https://openreview.net/pdf?id=Ee277P3AYC}.
        
        \bibitem[Boecking et~al.(2022)Boecking, Usuyama, Bannur, Castro, Schwaighofer, Hyland, Wetscherek, Naumann, Nori, Alvarez-Valle, et~al.]{boecking2022making}
        Benedikt Boecking, Naoto Usuyama, Shruthi Bannur, Daniel~C Castro, Anton Schwaighofer, Stephanie Hyland, Maria Wetscherek, Tristan Naumann, Aditya Nori, Javier Alvarez-Valle, et~al.
        \newblock Making the most of text semantics to improve biomedical vision--language processing.
        \newblock In \emph{European conference on computer vision}, pages 1--21. Springer, 2022.
        
        \bibitem[Huang et~al.(2021)Huang, Shen, Lungren, and Yeung]{huang2021gloria}
        Shih-Cheng Huang, Liyue Shen, Matthew~P Lungren, and Serena Yeung.
        \newblock Gloria: A multimodal global-local representation learning framework for label-efficient medical image recognition.
        \newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision}, pages 3942--3951, 2021.
        
        \bibitem[Zhang et~al.(2022)Zhang, Jiang, Miura, Manning, and Langlotz]{zhang2022contrastive}
        Yuhao Zhang, Hang Jiang, Yasuhide Miura, Christopher~D Manning, and Curtis~P Langlotz.
        \newblock Contrastive learning of medical visual representations from paired images and text.
        \newblock In \emph{Machine Learning for Healthcare Conference}, pages 2--25. PMLR, 2022.
        
        \bibitem[Zhou et~al.(2023)Zhou, Lian, Wang, and Yu]{zhou2023advancing}
        Hong-Yu Zhou, Chenyu Lian, Liansheng Wang, and Yizhou Yu.
        \newblock Advancing radiograph representation learning with masked record modeling.
        \newblock In \emph{The Eleventh International Conference on Learning Representations}, 2023.
        
        \bibitem[Li et~al.(2023)Li, Wong, Zhang, Usuyama, Liu, Yang, Naumann, Poon, and Gao]{li2023llava}
        Chunyuan Li, Cliff Wong, Sheng Zhang, Naoto Usuyama, Haotian Liu, Jianwei Yang, Tristan Naumann, Hoifung Poon, and Jianfeng Gao.
        \newblock Llava-med: Training a large language-and-vision assistant for biomedicine in one day.
        \newblock {\em Advances in Neural Information Processing Systems}, 36, 2024. 
        
        \bibitem[Moor et~al.(2023{\natexlab{a}})Moor, Huang, Wu, Yasunaga, Zakka, Dalmia, Reis, Rajpurkar, and Leskovec]{moor2023med}
        Michael Moor, Qian Huang, Shirley Wu, Michihiro Yasunaga, Cyril Zakka, Yash Dalmia, Eduardo~Pontes Reis, Pranav Rajpurkar, and Jure Leskovec.
        \newblock Med-flamingo: a multimodal medical few-shot learner.
        \newblock In {\em Machine Learning for Health (ML4H)}, pages 353--367. PMLR, 2023. 
        
        \bibitem[Tu et~al.(2023)Tu, Azizi, Driess, Schaekermann, Amin, Chang, Carroll, Lau, Tanno, Ktena, et~al.]{tu2023towards}
        Tao Tu, Shekoofeh Azizi, Danny Driess, Mike Schaekermann, Mohamed Amin, Pi-Chuan Chang, Andrew Carroll, Chuck Lau, Ryutaro Tanno, Ira Ktena, et~al.
        \newblock Towards generalist biomedical ai.
        \newblock {\em NEJM AI}, 1(3):AIoa2300138, 2024. Massachusetts Medical Society.  
        
        \bibitem[Moor et~al.(2023{\natexlab{b}})Moor, Banerjee, Abad, Krumholz, Leskovec, Topol, and Rajpurkar]{moor2023foundation}
        Michael Moor, Oishi Banerjee, Zahra Shakeri~Hossein Abad, Harlan~M Krumholz, Jure Leskovec, Eric~J Topol, and Pranav Rajpurkar.
        \newblock Foundation models for generalist medical artificial intelligence.
        \newblock \emph{Nature}, 616\penalty0 (7956):\penalty0 259--265, 2023{\natexlab{b}}.
        
        \bibitem[Dehghani et~al.(2023)Dehghani, Djolonga, Mustafa, Padlewski, Heek, Gilmer, Steiner, Caron, Geirhos, Alabdulmohsin, et~al.]{dehghani2023scaling}
        Mostafa Dehghani, Josip Djolonga, Basil Mustafa, Piotr Padlewski, Jonathan Heek, Justin Gilmer, Andreas~Peter Steiner, Mathilde Caron, Robert Geirhos, Ibrahim Alabdulmohsin, et~al.
        \newblock Scaling vision transformers to 22 billion parameters.
        \newblock In \emph{International Conference on Machine Learning}, pages 7480--7512. PMLR, 2023.
        
        \bibitem[Zhai et~al.(2022{\natexlab{a}})Zhai, Kolesnikov, Houlsby, and Beyer]{zhai2022scaling}
        Xiaohua Zhai, Alexander Kolesnikov, Neil Houlsby, and Lucas Beyer.
        \newblock Scaling vision transformers.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 12104--12113, 2022{\natexlab{a}}.
        
        \bibitem[Yang et~al.(2022)Yang, Duan, Tran, Xu, Chanda, Chen, Zeng, Chilimbi, and Huang]{yang2022vision}
        Jinyu Yang, Jiali Duan, Son Tran, Yi~Xu, Sampath Chanda, Liqun Chen, Belinda Zeng, Trishul Chilimbi, and Junzhou Huang.
        \newblock Vision-language pre-training with triple contrastive learning.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15671--15680, 2022.
        
        \bibitem[Zhai et~al.(2022{\natexlab{b}})Zhai, Wang, Mustafa, Steiner, Keysers, Kolesnikov, and Beyer]{zhai2022lit}
        Xiaohua Zhai, Xiao Wang, Basil Mustafa, Andreas Steiner, Daniel Keysers, Alexander Kolesnikov, and Lucas Beyer.
        \newblock Lit: Zero-shot transfer with locked-image text tuning.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 18123--18133, 2022{\natexlab{b}}.
        
        \bibitem[Liang et~al.(2022)Liang, Zhang, Kwon, Yeung, and Zou]{liang2022mind}
        Victor~Weixin Liang, Yuhui Zhang, Yongchan Kwon, Serena Yeung, and James~Y Zou.
        \newblock Mind the gap: Understanding the modality gap in multi-modal contrastive representation learning.
        \newblock \emph{Advances in Neural Information Processing Systems}, 35:\penalty0 17612--17625, 2022.
        
        \bibitem[Johnson et~al.(2019)Johnson, Pollard, Berkowitz, Greenbaum, Lungren, Deng, Mark, and Horng]{johnson2019mimic}
        Alistair~EW Johnson, Tom~J Pollard, Seth~J Berkowitz, Nathaniel~R Greenbaum, Matthew~P Lungren, Chih-ying Deng, Roger~G Mark, and Steven Horng.
        \newblock {MIMIC-CXR}, a de-identified publicly available database of chest radiographs with free-text reports.
        \newblock \emph{Scientific data}, 6\penalty0 (1):\penalty0 317, 2019.
        \newblock URL \url{https://physionet.org/content/mimic-cxr/2.0.0/}.
        
        \bibitem[Oord et~al.(2018)Oord, Li, and Vinyals]{oord2018representation}
        Aaron van~den Oord, Yazhe Li, and Oriol Vinyals.
        \newblock Representation learning with contrastive predictive coding.
        \newblock \emph{arXiv preprint arXiv:1807.03748}, 2018.
        \newblock URL \url{https://arxiv.org/pdf/1807.03748.pdf}.
        
        \bibitem[Chen et~al.(2020)Chen, Kornblith, Norouzi, and Hinton]{chen2020simple}
        Ting Chen, Simon Kornblith, Mohammad Norouzi, and Geoffrey Hinton.
        \newblock A simple framework for contrastive learning of visual representations.
        \newblock In \emph{International conference on machine learning}, pages 1597--1607. PMLR, 2020.
        \newblock URL \url{https://proceedings.mlr.press/v119/chen20j/chen20j.pdf}.
        
        \bibitem[Acosta et~al.(2022)Acosta, Falcone, Rajpurkar, and Topol]{acosta2022multimodal}
        Juli{\'a}n~N Acosta, Guido~J Falcone, Pranav Rajpurkar, and Eric~J Topol.
        \newblock Multimodal biomedical ai.
        \newblock \emph{Nature Medicine}, 28\penalty0 (9):\penalty0 1773--1784, 2022.
        
        \bibitem[Langlotz(2023)]{langlotz2023future}
        Curtis~P Langlotz.
        \newblock The future of ai and informatics in radiology: 10 predictions, 2023.
        
        \bibitem[Oquab et~al.(2024)Oquab, Darcet, Moutakanni, Vo, Szafraniec, Khalidov, Fernandez, HAZIZA, Massa, El-Nouby, Assran, Ballas, Galuba, Howes, Huang, Li, Misra, Rabbat, Sharma, Synnaeve, Xu, Jegou, Mairal, Labatut, Joulin, and Bojanowski]{oquab2023dinov2}
        Maxime Oquab, Timoth{\'e}e Darcet, Th{\'e}o Moutakanni, Huy~V. Vo, Marc Szafraniec, Vasil Khalidov, Pierre Fernandez, Daniel HAZIZA, Francisco Massa, Alaaeldin El-Nouby, Mido Assran, Nicolas Ballas, Wojciech Galuba, Russell Howes, Po-Yao Huang, Shang-Wen Li, Ishan Misra, Michael Rabbat, Vasu Sharma, Gabriel Synnaeve, Hu~Xu, Herve Jegou, Julien Mairal, Patrick Labatut, Armand Joulin, and Piotr Bojanowski.
        \newblock {DINO}v2: Learning robust visual features without supervision.
        \newblock \emph{Transactions on Machine Learning Research}, 2024.
        \newblock ISSN 2835-8856.
        \newblock URL \url{https://openreview.net/forum?id=a68SUt6zFt}.
        
        \bibitem[Huang et~al.(2023)Huang, Jin, Lu, Hou, Cheng, Fu, Shen, and Feng]{huang2023contrastive}
        Zhicheng Huang, Xiaojie Jin, Chengze Lu, Qibin Hou, Ming-Ming Cheng, Dongmei Fu, Xiaohui Shen, and Jiashi Feng.
        \newblock Contrastive masked autoencoders are stronger vision learners.
        \newblock \emph{IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2023.
        
        \bibitem[Park et~al.(2023)Park, Kim, Heo, Kim, and Yun]{park2023selfsupervised}
        Namuk Park, Wonjae Kim, Byeongho Heo, Taekyung Kim, and Sangdoo Yun.
        \newblock What do self-supervised vision transformers learn?
        \newblock In \emph{The Eleventh International Conference on Learning Representations}, 2023.
        
        \bibitem[Shekhar et~al.(2023)Shekhar, Bordes, Vincent, and Morcos]{shekhar2023objectives}
        Shashank Shekhar, Florian Bordes, Pascal Vincent, and Ari~S Morcos.
        \newblock Objectives matter: Understanding the impact of self-supervised objectives on vision transformer representations.
        \newblock In \emph{ICLR 2023 Workshop on Mathematical and Empirical Understanding of Foundation Models}, 2023.
        
        \bibitem[Ronneberger et~al.(2015)Ronneberger, Fischer, and Brox]{ronneberger2015u}
        Olaf Ronneberger, Philipp Fischer, and Thomas Brox.
        \newblock U-net: Convolutional networks for biomedical image segmentation.
        \newblock In \emph{Medical Image Computing and Computer-Assisted Intervention--MICCAI 2015: 18th International Conference, Munich, Germany, October 5-9, 2015, Proceedings, Part III 18}, pages 234--241. Springer, 2015.
        
        \bibitem[Liu et~al.(2021)Liu, Lin, Cao, Hu, Wei, Zhang, Lin, and Guo]{liu2021swin}
        Ze~Liu, Yutong Lin, Yue Cao, Han Hu, Yixuan Wei, Zheng Zhang, Stephen Lin, and Baining Guo.
        \newblock Swin transformer: Hierarchical vision transformer using shifted windows.
        \newblock In \emph{Proceedings of the IEEE/CVF international conference on computer vision}, pages 10012--10022, 2021.
        
        \bibitem[Li et~al.(2022)Li, Mao, Girshick, and He]{li2022exploring}
        Yanghao Li, Hanzi Mao, Ross Girshick, and Kaiming He.
        \newblock Exploring plain vision transformer backbones for object detection.
        \newblock In \emph{European Conference on Computer Vision}, pages 280--296. Springer, 2022.
        
        \bibitem[Xiao et~al.(2018)Xiao, Liu, Zhou, Jiang, and Sun]{xiao2018unified}
        Tete Xiao, Yingcheng Liu, Bolei Zhou, Yuning Jiang, and Jian Sun.
        \newblock Unified perceptual parsing for scene understanding.
        \newblock In \emph{Proceedings of the European conference on computer vision (ECCV)}, pages 418--434, 2018.
        \newblock URL \url{https://openaccess.thecvf.com/content_ECCV_2018/papers/Tete_Xiao_Unified_Perceptual_Parsing_ECCV_2018_paper.pdf}.
        
        \bibitem[Zhou et~al.(2019)Zhou, Sodha, Rahman~Siddiquee, Feng, Tajbakhsh, Gotway, and Liang]{zhou2019models}
        Zongwei Zhou, Vatsal Sodha, Md~Mahfuzur Rahman~Siddiquee, Ruibin Feng, Nima Tajbakhsh, Michael~B Gotway, and Jianming Liang.
        \newblock Models genesis: Generic autodidactic models for 3d medical image analysis.
        \newblock In \emph{Medical Image Computing and Computer Assisted Intervention--MICCAI 2019: 22nd International Conference, Shenzhen, China, October 13--17, 2019, Proceedings, Part IV 22}, pages 384--393. Springer, 2019.
        
        \bibitem[Tang et~al.(2022)Tang, Yang, Li, Roth, Landman, Xu, Nath, and Hatamizadeh]{tang2022self}
        Yucheng Tang, Dong Yang, Wenqi Li, Holger~R Roth, Bennett Landman, Daguang Xu, Vishwesh Nath, and Ali Hatamizadeh.
        \newblock Self-supervised pre-training of swin transformers for 3d medical image analysis.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 20730--20740, 2022.
        
        \bibitem[Assran et~al.(2023)Assran, Duval, Misra, Bojanowski, Vincent, Rabbat, LeCun, and Ballas]{assran2023self}
        Mahmoud Assran, Quentin Duval, Ishan Misra, Piotr Bojanowski, Pascal Vincent, Michael Rabbat, Yann LeCun, and Nicolas Ballas.
        \newblock Self-supervised learning from images with a joint-embedding predictive architecture.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15619--15629, 2023.
        
        \bibitem[Caron et~al.(2021)Caron, Touvron, Misra, J{\'e}gou, Mairal, Bojanowski, and Joulin]{caron2021emerging}
        Mathilde Caron, Hugo Touvron, Ishan Misra, Herv{\'e} J{\'e}gou, Julien Mairal, Piotr Bojanowski, and Armand Joulin.
        \newblock Emerging properties in self-supervised vision transformers.
        \newblock In \emph{Proceedings of the IEEE/CVF international conference on computer vision}, pages 9650--9660, 2021.
        
        \bibitem[Zhou et~al.(2022)Zhou, Wei, Wang, Shen, Xie, Yuille, and Kong]{zhou2022image}
        Jinghao Zhou, Chen Wei, Huiyu Wang, Wei Shen, Cihang Xie, Alan Yuille, and Tao Kong.
        \newblock {iBOT:} image {BERT} pre-training with online tokenizer.
        \newblock In \emph{International Conference on Learning Representations}, 2022.
        
        \bibitem[Xie et~al.(2023)Xie, Zhang, Cao, Lin, Wei, Dai, and Hu]{xie2023data}
        Zhenda Xie, Zheng Zhang, Yue Cao, Yutong Lin, Yixuan Wei, Qi~Dai, and Han Hu.
        \newblock On data scaling in masked image modeling.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 10365--10374, 2023.
        
        \bibitem[Zhang et~al.(2023{\natexlab{a}})Zhang, Xu, Usuyama, Bagga, Tinn, Preston, Rao, Wei, Valluri, Wong, et~al.]{zhang2023large}
        Sheng Zhang, Yanbo Xu, Naoto Usuyama, Jaspreet Bagga, Robert Tinn, Sam Preston, Rajesh Rao, Mu~Wei, Naveen Valluri, Cliff Wong, et~al.
        \newblock Large-scale domain-specific pretraining for biomedical vision-language processing.
        \newblock \emph{arXiv preprint arXiv:2303.00915}, 2023{\natexlab{a}}.
        \newblock URL \url{https://arxiv.org/pdf/2303.00915.pdf}.
        
        \bibitem[Cherti and Jitsev(2022)]{cherti2022effect}
        Mehdi Cherti and Jenia Jitsev.
        \newblock Effect of pre-training scale on intra-and inter-domain, full and few-shot transfer learning for natural and x-ray chest images.
        \newblock In \emph{2022 International Joint Conference on Neural Networks (IJCNN)}, pages 1--9. IEEE, 2022.
        \newblock URL \url{https://arxiv.org/pdf/2106.00116.pdf}.
        
        \bibitem[Mustafa et~al.(2021)Mustafa, Loh, Freyberg, MacWilliams, Wilson, McKinney, Sieniek, Winkens, Liu, Bui, et~al.]{mustafa2021supervised}
        Basil Mustafa, Aaron Loh, Jan Freyberg, Patricia MacWilliams, Megan Wilson, Scott~Mayer McKinney, Marcin Sieniek, Jim Winkens, Yuan Liu, Peggy Bui, et~al.
        \newblock Supervised transfer learning at scale for medical imaging.
        \newblock \emph{arXiv preprint arXiv:2101.05913}, 2021.
        \newblock URL \url{https://arxiv.org/pdf/2101.05913.pdf}.
        
        \bibitem[Bertrand et~al.(2019)Bertrand, Hashir, and Cohen]{bertrand2019lateral}
        Hadrien Bertrand, Mohammad Hashir, and Joseph~Paul Cohen.
        \newblock Do lateral views help automated chest x-ray predictions?
        \newblock In {\em MIDL Abstract}, 2019. 
        
        \bibitem[Hashir et~al.(2020)Hashir, Bertrand, and Cohen]{hashir2020quantifying}
        Mohammad Hashir, Hadrien Bertrand, and Joseph~Paul Cohen.
        \newblock Quantifying the value of lateral views in deep learning for chest x-rays.
        \newblock In \emph{Medical Imaging with Deep Learning}, pages 288--303. PMLR, 2020.
        \newblock URL \url{https://proceedings.mlr.press/v121/hashir20a/hashir20a.pdf}.
        
        \bibitem[Caron et~al.(2020)Caron, Misra, Mairal, Goyal, Bojanowski, and Joulin]{caron2020unsupervised}
        Mathilde Caron, Ishan Misra, Julien Mairal, Priya Goyal, Piotr Bojanowski, and Armand Joulin.
        \newblock Unsupervised learning of visual features by contrasting cluster assignments.
        \newblock \emph{Advances in neural information processing systems}, 33:\penalty0 9912--9924, 2020.
        
        \bibitem[Demner-Fushman et~al.(2016)Demner-Fushman, Kohli, Rosenman, Shooshan, Rodriguez, Antani, Thoma, and McDonald]{demner2016preparing}
        Dina Demner-Fushman, Marc~D Kohli, Marc~B Rosenman, Sonya~E Shooshan, Laritza Rodriguez, Sameer Antani, George~R Thoma, and Clement~J McDonald.
        \newblock Preparing a collection of radiology examinations for distribution and retrieval.
        \newblock \emph{Journal of the American Medical Informatics Association}, 23\penalty0 (2):\penalty0 304--310, 2016.
        
        \bibitem[Liu et~al.(2023{\natexlab{a}})Liu, Li, Wu, and Lee]{liu_visual_2023}
        Haotian Liu, Chunyuan Li, Qingyang Wu, and Yong~Jae Lee.
        \newblock {\em Advances in Neural Information Processing Systems}, 36, 2024. 
        
        \bibitem[Liu et~al.(2023{\natexlab{b}})Liu, Li, Li, and Lee]{liu_improved_2023}
        Haotian Liu, Chunyuan Li, Yuheng Li, and Yong~Jae Lee.
        \newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 26296--26306, 2024.  
        
        \bibitem[Chiang et~al.(2023)Chiang, Li, Lin, Sheng, Wu, Zhang, Zheng, Zhuang, Zhuang, Gonzalez, Stoica, and Xing]{vicuna2023}
        Wei-Lin Chiang, Zhuohan Li, Zi~Lin, Ying Sheng, Zhanghao Wu, Hao Zhang, Lianmin Zheng, Siyuan Zhuang, Yonghao Zhuang, Joseph~E. Gonzalez, Ion Stoica, and Eric~P. Xing.
        \newblock Vicuna: An open-source chatbot impressing gpt-4 with 90\%* chatgpt quality, March 2023.
        \newblock URL \url{https://lmsys.org/blog/2023-03-30-vicuna/}.
        
        \bibitem[Yang et~al.(2023)Yang, Cherian, and Vucetic]{yang2023data}
        Ziyu Yang, Santhosh Cherian, and Slobodan Vucetic.
        \newblock Data augmentation for radiology report simplification.
        \newblock In \emph{Findings of the Association for Computational Linguistics: EACL 2023}, pages 1877--1887, 2023.
        
        \bibitem[Bannur et~al.(2023)Bannur, Hyland, Liu, Perez-Garcia, Ilse, Castro, Boecking, Sharma, Bouzid, Thieme, et~al.]{bannur2023learning}
        Shruthi Bannur, Stephanie Hyland, Qianchu Liu, Fernando Perez-Garcia, Maximilian Ilse, Daniel~C Castro, Benedikt Boecking, Harshita Sharma, Kenza Bouzid, Anja Thieme, et~al.
        \newblock Learning to exploit temporal structure for biomedical vision-language processing.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15016--15027, 2023.
        
        \bibitem[Lin(2004)]{lin_rouge_2004}
        Chin-Yew Lin.
        \newblock {ROUGE}: A package for automatic evaluation of summaries.
        \newblock In \emph{Text {Summarization} {Branches} {Out}}, pages 74--81. Association for Computational Linguistics, July 2004.
        \newblock URL \url{https://aclanthology.org/W04-1013}.
        
        \bibitem[Papineni et~al.(2002)Papineni, Roukos, Ward, and Zhu]{papineni_bleu_2002}
        Kishore Papineni, Salim Roukos, Todd Ward, and Wei-Jing Zhu.
        \newblock {BLEU}: a method for automatic evaluation of machine translation.
        \newblock In \emph{Proceedings of the 40th {Annual} {Meeting} of the {Association} for {Computational} {Linguistics}}, pages 311--318. Association for Computational Linguistics, July 2002.
        \newblock \doi{10.3115/1073083.1073135}.
        
        \bibitem[Delbrouck et~al.(2022)Delbrouck, Chambon, Bluethgen, Tsai, Almusa, and Langlotz]{semantic_rewards}
        Jean-Benoit Delbrouck, Pierre Chambon, Christian Bluethgen, Emily Tsai, Omar Almusa, and Curtis Langlotz.
        \newblock Improving the factual correctness of radiology report generation with semantic rewards.
        \newblock In \emph{Findings of the {Association} for {Computational} {Linguistics}: {EMNLP} 2022}, pages 4348--4360. ACL, December 2022.
        \newblock \doi{10.18653/v1/2022.findings-emnlp.319}.
        
        \bibitem[Smit et~al.(2020)Smit, Jain, Rajpurkar, Pareek, Ng, and Lungren]{chexbert}
        Akshay Smit, Saahil Jain, Pranav Rajpurkar, Anuj Pareek, Andrew Ng, and Matthew Lungren.
        \newblock Combining automatic labelers and expert annotations for accurate radiology report labeling using {BERT}.
        \newblock In \emph{Proceedings of the 2020 Conference on Empirical Methods in Natural Language Processing (EMNLP)}, pages 1500--1519. ACL, November 2020.
        \newblock \doi{10.18653/v1/2020.emnlp-main.117}.
        
        \bibitem[Irvin et~al.(2019)Irvin, Rajpurkar, Ko, Yu, Ciurea-Ilcus, Chute, Marklund, Haghgoo, Ball, Shpanskaya, Seekins, Mong, Halabi, Sandberg, Jones, Larson, Langlotz, Patel, Lungren, and Ng]{chexpert}
        Jeremy Irvin, Pranav Rajpurkar, Michael Ko, Yifan Yu, Silviana Ciurea-Ilcus, Chris Chute, Henrik Marklund, Behzad Haghgoo, Robyn~L. Ball, Katie Shpanskaya, Jayne Seekins, David~A. Mong, Safwan~S. Halabi, Jesse~K. Sandberg, Ricky Jones, David~B. Larson, Curtis~P. Langlotz, Bhavik~N. Patel, Matthew~P. Lungren, and Andrew~Y. Ng.
        \newblock {CheXpert}: A large chest radiograph dataset with uncertainty labels and expert comparison.
        \newblock In \emph{Proceedings of the {AAAI} {Conference} on {Artificial} {Intelligence} ({AAAI} 2019)}, volume~33, pages 590--597. AAAI Press, July 2019.
        \newblock \doi{10.1609/aaai.v33i01.3301590}.
        
        \bibitem[Lin et~al.(2023{\natexlab{a}})Lin, Yin, Ping, Lu, Molchanov, Tao, Mao, Kautz, Shoeybi, and Han]{lin2023vila}
        Ji~Lin, Hongxu Yin, Wei Ping, Yao Lu, Pavlo Molchanov, Andrew Tao, Huizi Mao, Jan Kautz, Mohammad Shoeybi, and Song Han.
        \newblock Vila: On pre-training for visual language models.
        \newblock In {\em Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 26689--26699, 2024.  
        
        \bibitem[Lin et~al.(2017)Lin, Doll{\'a}r, Girshick, He, Hariharan, and Belongie]{lin2017feature}
        Tsung-Yi Lin, Piotr Doll{\'a}r, Ross Girshick, Kaiming He, Bharath Hariharan, and Serge Belongie.
        \newblock Feature pyramid networks for object detection.
        \newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 2117--2125, 2017.
        
        \bibitem[Azad et~al.(2022)Azad, Aghdam, Rauland, Jia, Avval, Bozorgpour, Karimijafarbigloo, Cohen, Adeli, and Merhof]{azad2022medical}
        Reza Azad, Ehsan~Khodapanah Aghdam, Amelie Rauland, Yiwei Jia, Atlas~Haddadi Avval, Afshin Bozorgpour, Sanaz Karimijafarbigloo, Joseph~Paul Cohen, Ehsan Adeli, and Dorit Merhof.
        \newblock Medical image segmentation review: The success of u-net.
        \newblock {\em IEEE Transactions on Pattern Analysis and Machine Intelligence}, 2024. IEEE.  
        
        \bibitem[Isensee et~al.(2018)Isensee, Petersen, Klein, Zimmerer, Jaeger, Kohl, Wasserthal, Koehler, Norajitra, Wirkert, and Maier-Hein]{isensee2018nnunet}
        Fabian Isensee, Jens Petersen, Andre Klein, David Zimmerer, Paul~F. Jaeger, Simon Kohl, Jakob Wasserthal, Gregor Koehler, Tobias Norajitra, Sebastian Wirkert, and Klaus~H. Maier-Hein.
        \newblock nnu-net: Self-adapting framework for u-net-based medical image segmentation.
        \newblock {\em Nature Methods}, 18:203--211, 2021. 
        
        \bibitem[Tan and Le(2020)]{tan2020efficientnet}
        Mingxing Tan and Quoc~V. Le.
        \newblock Efficientnet: Rethinking model scaling for convolutional neural networks.
        \newblock In {\em International Conference on Machine Learning}, pages 6105--6114. PMLR, 2019. 
        
        \bibitem[Ilharco et~al.(2022)Ilharco, Wortsman, Wightman, Gordon, Carlini, Taori, Dave, Shankar, Namkoong, Miller, Hajishirzi, Farhadi, and Schmidt]{ilharco_2022_7086307}
        Gabriel Ilharco, Mitchell Wortsman, Ross Wightman, Cade Gordon, Nicholas Carlini, Rohan Taori, Achal Dave, Vaishaal Shankar, Hongseok Namkoong, John Miller, Hannaneh Hajishirzi, Ali Farhadi, and Ludwig Schmidt.
        \newblock {OpenCLIP}, September 2022.
        \newblock URL \url{https://doi.org/10.5281/zenodo.7086307}.
        
        \bibitem[Wang et~al.(2024)Wang, Zhang, Feng, Cascone, Nappi, and Wan]{wang2024multi}
        Hongyu Wang, Dandan Zhang, Jun Feng, Lucia Cascone, Michele Nappi, and Shaohua Wan.
        \newblock A multi-objective segmentation method for chest x-rays based on collaborative learning from multiple partially annotated datasets.
        \newblock \emph{Information Fusion}, 102:\penalty0 102016, 2024.
        
        \bibitem[Zhang et~al.(2023{\natexlab{b}})Zhang, Wang, Deng, Wang, Shen, and Feng]{zhang2023cams}
        Dandan Zhang, Hongyu Wang, Jiahui Deng, Tonghui Wang, Cong Shen, and Jun Feng.
        \newblock Cams-net: An attention-guided feature selection network for rib segmentation in chest x-rays.
        \newblock \emph{Computers in Biology and Medicine}, 156:\penalty0 106702, 2023{\natexlab{b}}.
        
        \bibitem[Pal et~al.(2023)Pal, Meena, and Roy]{pal2023fully}
        Debojyoti Pal, Tanushree Meena, and Sudipta Roy.
        \newblock A fully connected reproducible se-uresnet for multiorgan chest radiographs segmentation.
        \newblock In \emph{2023 IEEE 24th International Conference on Information Reuse and Integration for Data Science (IRI)}, pages 261--266. IEEE, 2023.
        
        \bibitem[Brioso et~al.(2023)Brioso, Pedrosa, Mendon{\c{c}}a, and Campilho]{brioso2023semi}
        Ricardo~Coimbra Brioso, Jo{\~a}o Pedrosa, Ana~Maria Mendon{\c{c}}a, and Aur{\'e}lio Campilho.
        \newblock Semi-supervised multi-structure segmentation in chest x-ray imaging.
        \newblock In \emph{2023 IEEE 36th International Symposium on Computer-Based Medical Systems (CBMS)}, pages 814--820. IEEE, 2023.
        
        \bibitem[Boos et~al.(2016)Boos, Lanzman, Heusch, Aissa, Schleich, Thomas, Sawicki, Antoch, and Kr{\"o}pil]{boos2016does}
        Johannes Boos, Rotem~S Lanzman, Philipp Heusch, Joel Aissa, Christoph Schleich, Christoph Thomas, Lino~M Sawicki, Gerald Antoch, and Patric Kr{\"o}pil.
        \newblock Does body mass index outperform body weight as a surrogate parameter in the calculation of size-specific dose estimates in adult body ct?
        \newblock \emph{The British Journal of Radiology}, 89\penalty0 (1059):\penalty0 20150734, 2016.
        
        \bibitem[Demircio{\u{g}}lu et~al.(2023)Demircio{\u{g}}lu, Quinsten, Umutlu, Forsting, Nassenstein, and Bos]{demirciouglu2023determining}
        Aydin Demircio{\u{g}}lu, Anton~S Quinsten, Lale Umutlu, Michael Forsting, Kai Nassenstein, and Denise Bos.
        \newblock Determining body height and weight from thoracic and abdominal ct localizers in pediatric and young adult patients using deep learning.
        \newblock \emph{Scientific Reports}, 13\penalty0 (1):\penalty0 19010, 2023.
        
        \bibitem[Ichikawa et~al.(2021)Ichikawa, Hamada, and Sugimori]{ichikawa2021deep}
        Shota Ichikawa, Misaki Hamada, and Hiroyuki Sugimori.
        \newblock A deep-learning method using computed tomography scout images for estimating patient body weight.
        \newblock \emph{Scientific reports}, 11\penalty0 (1):\penalty0 15627, 2021.
        
        \bibitem[Johnson et~al.(2023)Johnson, Bulgarelli, Pollard, Horng, Celi, and Mark]{mimiciv_v2}
        Alistair Johnson, Lucas Bulgarelli, Tom Pollard, Steven Horng, Leo~Anthony Celi, and Roger Mark.
        \newblock Mimic-iv, 2023.
        \newblock URL \url{https://physionet.org/content/mimiciv/2.2/}.
        
        \bibitem[Huix et~al.(2024)Huix, Ganeshan, Haslum, S{\"o}derberg, Matsoukas, and Smith]{huix2024natural}
        Joana~Pal{\'e}s Huix, Adithya~Raju Ganeshan, Johan~Fredin Haslum, Magnus S{\"o}derberg, Christos Matsoukas, and Kevin Smith.
        \newblock Are natural domain foundation models useful for medical image classification?
        \newblock In \emph{Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision}, pages 7634--7643, 2024.
        
        \bibitem[Wan et~al.(2023)Wan, Liu, Zhang, Fu, Wang, Cheng, Ma, Quilodr'an-Casas, and Arcucci]{Wan2023MedUniCUC}
        Zhongwei Wan, Che Liu, Mi~Zhang, Jie Fu, Benyou Wang, Sibo Cheng, Lei Ma, Cesar~C'esar Quilodr'an-Casas, and Rossella Arcucci.
        \newblock Med-unic: Unifying cross-lingual medical vision-language pre-training by diminishing bias.
        \newblock \emph{Advances in Neural Information Processing Systems}, 2023.
        
        \bibitem[Brown et~al.(2020)Brown, Mann, Ryder, Subbiah, Kaplan, Dhariwal, Neelakantan, Shyam, Sastry, Askell, et~al.]{brown2020language}
        Tom Brown, Benjamin Mann, Nick Ryder, Melanie Subbiah, Jared~D Kaplan, Prafulla Dhariwal, Arvind Neelakantan, Pranav Shyam, Girish Sastry, Amanda Askell, et~al.
        \newblock Language models are few-shot learners.
        \newblock \emph{Advances in neural information processing systems}, 33:\penalty0 1877--1901, 2020.
        
        \bibitem[Achiam et~al.(2023)Achiam, Adler, Agarwal, Ahmad, Akkaya, Aleman, Almeida, Altenschmidt, Altman, Anadkat, et~al.]{achiam2023gpt}
        Josh Achiam, Steven Adler, Sandhini Agarwal, Lama Ahmad, Ilge Akkaya, Florencia~Leoni Aleman, Diogo Almeida, Janko Altenschmidt, Sam Altman, Shyamal Anadkat, et~al.
        \newblock Gpt-4 technical report.
        \newblock \emph{arXiv preprint arXiv:2303.08774}, 2023.
        \newblock URL \url{https://arxiv.org/pdf/2303.08774.pdf}.
        
        \bibitem[Nori et~al.(2023)Nori, Lee, Zhang, Carignan, Edgar, Fusi, King, Larson, Li, Liu, et~al.]{nori2023can}
        Harsha Nori, Yin~Tat Lee, Sheng Zhang, Dean Carignan, Richard Edgar, Nicolo Fusi, Nicholas King, Jonathan Larson, Yuanzhi Li, Weishung Liu, et~al.
        \newblock Can generalist foundation models outcompete special-purpose tuning? case study in medicine.
        \newblock \emph{arXiv preprint arXiv:2311.16452}, 2023.
        \newblock URL \url{https://arxiv.org/pdf/2311.16452.pdf}.
        
        \bibitem[Jiang et~al.(2023)Jiang, Liu, Liu, Zhang, Li, Xiong, and Tian]{jiang2023clip}
        Dongsheng Jiang, Yuchen Liu, Songlin Liu, Xiaopeng Zhang, Jin Li, Hongkai Xiong, and Qi~Tian.
        \newblock From clip to dino: Visual encoders shout in multi-modal large language models, 2023.
        \newblock URL \url{https://arxiv.org/pdf/2310.08825v1.pdf}.
        
        \bibitem[Wang et~al.(2017)Wang, Peng, Lu, Lu, Bagheri, and Summers]{wang2017chestx}
        Xiaosong Wang, Yifan Peng, Le~Lu, Zhiyong Lu, Mohammadhadi Bagheri, and Ronald~M Summers.
        \newblock Chestx-ray8: Hospital-scale chest x-ray database and benchmarks on weakly-supervised classification and localization of common thorax diseases.
        \newblock In \emph{Proceedings of the IEEE conference on computer vision and pattern recognition}, pages 2097--2106, 2017.
        
        \bibitem[Bustos et~al.(2020)Bustos, Pertusa, Salinas, and de~la Iglesia-Vayá]{Bustos_2020}
        Aurelia Bustos, Antonio Pertusa, Jose-Maria Salinas, and Maria de~la Iglesia-Vayá.
        \newblock {PadChest: A large chest x-ray image dataset with multi-label annotated reports}.
        \newblock \emph{Medical Image Analysis}, 66:\penalty0 101797, December 2020.
        \newblock ISSN 1361-8415.
        \newblock \doi{10.1016/j.media.2020.101797}.
        \newblock URL \url{http://dx.doi.org/10.1016/j.media.2020.101797}.
        
        \bibitem[Nguyen et~al.(2021)Nguyen, Le, Pham, and Nguyen]{nguyen2021vindrribcxr}
        Hoang~C. Nguyen, Tung~T. Le, Hieu~H. Pham, and Ha~Q. Nguyen.
        \newblock Vindr-ribcxr: A benchmark dataset for automatic segmentation and labeling of individual ribs on chest x-rays, 2021.
        \newblock In {\em Medical Imaging with Deep Learning}, 2021.  
        
        \bibitem[Feng et~al.(2021)Feng, Azzollini, Kim, Jin, Gordon, Yeoh, Kim, Han, Lee, Patel, et~al.]{feng2021curation}
        Sijing Feng, Damian Azzollini, Ji~Soo Kim, Cheng-Kai Jin, Simon~P Gordon, Jason Yeoh, Eve Kim, Mina Han, Andrew Lee, Aakash Patel, et~al.
        \newblock Curation of the candid-ptx dataset with free-text reports.
        \newblock \emph{Radiology: Artificial Intelligence}, 3\penalty0 (6):\penalty0 e210136, 2021.
        
        \bibitem[MD et~al.(2018)MD, Wu, Carr, Shih, Dulkowski, kalpathy, Chen, Prevedello, MD, McDonald, Peter, Culliton, MD, and Xia]{rsna-pneumonia-detection-challenge}
        Anouk~Stein MD, Carol Wu, Chris Carr, George Shih, Jamie Dulkowski, kalpathy, Leon Chen, Luciano Prevedello, Marc~Kohli MD, Mark McDonald, Peter, Phil Culliton, Safwan~Halabi MD, and Tian Xia.
        \newblock Rsna pneumonia detection challenge, 2018.
        \newblock URL \url{https://kaggle.com/competitions/rsna-pneumonia-detection-challenge}.
        
        \bibitem[Goldberger et~al.(2000)Goldberger, Amaral, Glass, Hausdorff, Ivanov, Mark, Mietus, Moody, Peng, and Stanley]{physionet}
        Ary~L. Goldberger, Luis A.~N. Amaral, Leon Glass, Jeffrey~M. Hausdorff, Plamen~Ch. Ivanov, Roger~G. Mark, Joseph~E. Mietus, George~B. Moody, Chung-Kang Peng, and H.~Eugene Stanley.
        \newblock Physiobank, physiotoolkit, and physionet.
        \newblock \emph{Circulation}, 101\penalty0 (23):\penalty0 e215--e220, 2000.
        \newblock \doi{10.1161/01.CIR.101.23.e215}.
        \newblock URL \url{https://www.ahajournals.org/doi/abs/10.1161/01.CIR.101.23.e215}.
        
        \bibitem[Nguyen et~al.(2022)Nguyen, Lam, Le, Pham, Tran, Nguyen, Le, Pham, Tong, Dinh, et~al.]{nguyen2020vindrcxr}
        Ha~Q Nguyen, Khanh Lam, Linh~T Le, Hieu~H Pham, Dat~Q Tran, Dung~B Nguyen, Dung~D Le, Chi~M Pham, Hang~TT Tong, Diep~H Dinh, et~al.
        \newblock Vindr-cxr: An open dataset of chest x-rays with radiologist’s annotations.
        \newblock \emph{Scientific Data}, 9\penalty0 (1):\penalty0 429, 2022.
        
        \bibitem[Wu et~al.(2021)Wu, Agu, Lourentzou, Sharma, Paguio, Yao, Dee, Mitchell, Kashyap, Giovannini, et~al.]{wu2021chest}
        Joy~T Wu, Nkechinyere~N Agu, Ismini Lourentzou, Arjun Sharma, Joseph~A Paguio, Jasper~S Yao, Edward~C Dee, William Mitchell, Satyananda Kashyap, Andrea Giovannini, et~al.
        \newblock Chest imagenome dataset (version 1.0. 0).
        \newblock \emph{PhysioNet}, 5:\penalty0 18, 2021.
        
        \bibitem[Reis et~al.(2022)Reis, de~Paiva, da~Silva, Ribeiro, Paiva, Bulgarelli, Lee, Santos, Brito, Amaral, et~al.]{reis2022brax}
        Eduardo~P Reis, Joselisa~PQ de~Paiva, Maria~CB da~Silva, Guilherme~AS Ribeiro, Victor~F Paiva, Lucas Bulgarelli, Henrique~MH Lee, Paulo~V Santos, Vanessa~M Brito, Lucas~TW Amaral, et~al.
        \newblock {BRAX, Brazilian labeled chest x-ray dataset}.
        \newblock \emph{Scientific Data}, 9\penalty0 (1):\penalty0 487, 2022.
        
        \bibitem[Chen et~al.(2022)Chen, Kuo, Wang, Gichoya, and Celi]{chen2022cxrmimic}
        Li-Ching Chen, Po-Chih Kuo, Ryan Wang, Judy Gichoya, and Leo~Anthony Celi.
        \newblock Chest x-ray segmentation images based on mimic-cxr, 2022.
        \newblock URL \url{https://physionet.org/content/lung-segment-mimic-cxr/1.0.0/}.
        
        \bibitem[Tiu et~al.(2022)Tiu, Talius, Patel, Langlotz, Ng, and Rajpurkar]{tiu2022expert}
        Ekin Tiu, Ellie Talius, Pujan Patel, Curtis~P Langlotz, Andrew~Y Ng, and Pranav Rajpurkar.
        \newblock Expert-level detection of pathologies from unannotated chest x-ray images via self-supervised learning.
        \newblock \emph{Nature Biomedical Engineering}, 6\penalty0 (12):\penalty0 1399--1406, 2022.
        
        \bibitem[Grill et~al.(2020)Grill, Strub, Altch{\'e}, Tallec, Richemond, Buchatskaya, Doersch, Avila~Pires, Guo, Gheshlaghi~Azar, et~al.]{grill2020bootstrap}
        Jean-Bastien Grill, Florian Strub, Florent Altch{\'e}, Corentin Tallec, Pierre Richemond, Elena Buchatskaya, Carl Doersch, Bernardo Avila~Pires, Zhaohan Guo, Mohammad Gheshlaghi~Azar, et~al.
        \newblock Bootstrap your own latent-a new approach to self-supervised learning.
        \newblock \emph{Advances in neural information processing systems}, 33:\penalty0 21271--21284, 2020.
        
        \bibitem[Chen and He(2021)]{chen2021exploring}
        Xinlei Chen and Kaiming He.
        \newblock Exploring simple siamese representation learning.
        \newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 15750--15758, 2021.
        
        \bibitem[Bao et~al.(2021)Bao, Dong, Piao, and Wei]{bao2021beit}
        Hangbo Bao, Li~Dong, Songhao Piao, and Furu Wei.
        \newblock Beit: Bert pre-training of image transformers.
        \newblock In \emph{International Conference on Learning Representations}, 2021.
        
        \bibitem[He et~al.(2022)He, Chen, Xie, Li, Doll{\'a}r, and Girshick]{he2022masked}
        Kaiming He, Xinlei Chen, Saining Xie, Yanghao Li, Piotr Doll{\'a}r, and Ross Girshick.
        \newblock Masked autoencoders are scalable vision learners.
        \newblock In \emph{Proceedings of the IEEE/CVF conference on computer vision and pattern recognition}, pages 16000--16009, 2022.
        
        \bibitem[Shen et~al.(2022)Shen, Li, Hu, Xie, Yang, Zhang, Gan, Wang, Yuan, Liu, et~al.]{shen2022k}
        Sheng Shen, Chunyuan Li, Xiaowei Hu, Yujia Xie, Jianwei Yang, Pengchuan Zhang, Zhe Gan, Lijuan Wang, Lu~Yuan, Ce~Liu, et~al.
        \newblock K-lite: Learning transferable visual models with external knowledge.
        \newblock \emph{Advances in Neural Information Processing Systems}, 35:\penalty0 15558--15573, 2022.
        
        \bibitem[Yao et~al.(2021)Yao, Huang, Hou, Lu, Niu, Xu, Liang, Li, Jiang, and Xu]{yao2021filip}
        Lewei Yao, Runhui Huang, Lu~Hou, Guansong Lu, Minzhe Niu, Hang Xu, Xiaodan Liang, Zhenguo Li, Xin Jiang, and Chunjing Xu.
        \newblock Filip: Fine-grained interactive language-image pre-training.
        \newblock In \emph{International Conference on Learning Representations}, 2021.
        
        \bibitem[Girdhar et~al.(2023)Girdhar, El-Nouby, Liu, Singh, Alwala, Joulin, and Misra]{girdhar2023imagebind}
        Rohit Girdhar, Alaaeldin El-Nouby, Zhuang Liu, Mannat Singh, Kalyan~Vasudev Alwala, Armand Joulin, and Ishan Misra.
        \newblock Imagebind: One embedding space to bind them all.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15180--15190, 2023.
        
        \bibitem[Yu et~al.(2022{\natexlab{b}})Yu, Wang, Vasudevan, Yeung, Seyedhosseini, and Wu]{yu2022coca}
        Jiahui Yu, Zirui Wang, Vijay Vasudevan, Legg Yeung, Mojtaba Seyedhosseini, and Yonghui Wu.
        \newblock Coca: Contrastive captioners are image-text foundation models.
        \newblock \emph{Transactions on Machine Learning Research}, 2022{\natexlab{b}}.
        \newblock ISSN 2835-8856.
        
        \bibitem[Wang et~al.(2022{\natexlab{a}})Wang, Yu, Yu, Dai, Tsvetkov, and Cao]{wang2022simvlm}
        Zirui Wang, Jiahui Yu, Adams~Wei Yu, Zihang Dai, Yulia Tsvetkov, and Yuan Cao.
        \newblock Sim{VLM}: Simple visual language model pretraining with weak supervision.
        \newblock In \emph{International Conference on Learning Representations}, 2022{\natexlab{a}}.
        
        \bibitem[Singh et~al.(2022)Singh, Hu, Goswami, Couairon, Galuba, Rohrbach, and Kiela]{singh2022flava}
        Amanpreet Singh, Ronghang Hu, Vedanuj Goswami, Guillaume Couairon, Wojciech Galuba, Marcus Rohrbach, and Douwe Kiela.
        \newblock Flava: A foundational language and vision alignment model.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 15638--15650, 2022.
        
        \bibitem[Tschannen et~al.(2023)Tschannen, Kumar, Steiner, Zhai, Houlsby, and Beyer]{tschannen2023image}
        Michael Tschannen, Manoj Kumar, Andreas Steiner, Xiaohua Zhai, Neil Houlsby, and Lucas Beyer.
        \newblock Image captioners are scalable vision learners too.
        \newblock {\em Advances in Neural Information Processing Systems}, 36, 2024. 
        
        \bibitem[Li et~al.(2021)Li, Liang, Zhao, Cui, Ouyang, Shao, Yu, and Yan]{li2021supervision}
        Yangguang Li, Feng Liang, Lichen Zhao, Yufeng Cui, Wanli Ouyang, Jing Shao, Fengwei Yu, and Junjie Yan.
        \newblock Supervision exists everywhere: A data efficient contrastive language-image pre-training paradigm.
        \newblock In \emph{International Conference on Learning Representations}, 2021.
        
        \bibitem[Weers et~al.(2023)Weers, Shankar, Katharopoulos, Yang, and Gunter]{weers2023masked}
        Floris Weers, Vaishaal Shankar, Angelos Katharopoulos, Yinfei Yang, and Tom Gunter.
        \newblock Masked autoencoding does not help natural language supervision at scale.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 23432--23444, 2023.
        
        \bibitem[Mu et~al.(2022)Mu, Kirillov, Wagner, and Xie]{mu2022slip}
        Norman Mu, Alexander Kirillov, David Wagner, and Saining Xie.
        \newblock Slip: Self-supervision meets language-image pre-training.
        \newblock In \emph{European Conference on Computer Vision}, pages 529--544. Springer, 2022.
        
        \bibitem[Wu et~al.(2023)Wu, Zhang, Zhang, Wang, and Xie]{Wu_2023_ICCV}
        Chaoyi Wu, Xiaoman Zhang, Ya~Zhang, Yanfeng Wang, and Weidi Xie.
        \newblock Medklip: Medical knowledge enhanced language-image pre-training for x-ray diagnosis.
        \newblock In \emph{Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)}, pages 21372--21383, October 2023.
        \newblock URL \url{https://openaccess.thecvf.com/content/ICCV2023/papers/Wu_MedKLIP_Medical_Knowledge_Enhanced_Language-Image_Pre-Training_for_X-ray_Diagnosis_ICCV_2023_paper.pdf}.
        
        \bibitem[Lin et~al.(2023{\natexlab{b}})Lin, Zhao, Zhang, Wu, Zhang, Wang, and Xie]{lin2023pmcclip}
        Weixiong Lin, Ziheng Zhao, Xiaoman Zhang, Chaoyi Wu, Ya~Zhang, Yanfeng Wang, and Weidi Xie.
        \newblock Pmc-clip: Contrastive language-image pre-training using biomedical documents.
        \newblock In {\em International Conference on Medical Image Computing and Computer-Assisted Intervention}, pages 525--536. Springer, 2023.  
        
        \bibitem[Wang et~al.(2022{\natexlab{b}})Wang, Wu, Agarwal, and Sun]{wang2022medclip}
        Zifeng Wang, Zhenbang Wu, Dinesh Agarwal, and Jimeng Sun.
        \newblock Medclip: Contrastive learning from unpaired medical images and text, 2022{\natexlab{b}}.
        \newblock In {\em Proceedings of the 2022 Conference on Empirical Methods in Natural Language Processing}, pages 3876--3887, 2022.  
        
        \bibitem[Alayrac et~al.(2022)Alayrac, Donahue, Luc, Miech, Barr, Hasson, Lenc, Mensch, Millican, Reynolds, et~al.]{alayrac2022flamingo}
        Jean-Baptiste Alayrac, Jeff Donahue, Pauline Luc, Antoine Miech, Iain Barr, Yana Hasson, Karel Lenc, Arthur Mensch, Katherine Millican, Malcolm Reynolds, et~al.
        \newblock Flamingo: a visual language model for few-shot learning.
        \newblock \emph{Advances in Neural Information Processing Systems}, 35:\penalty0 23716--23736, 2022.
        
        \bibitem[Park et~al.(2022)Park, Kim, Oh, Seo, Lee, Kim, Moon, Lim, Park, and Ye]{park2022self}
        Sangjoon Park, Gwanghyun Kim, Yujin Oh, Joon~Beom Seo, Sang~Min Lee, Jin~Hwan Kim, Sungjun Moon, Jae-Kwang Lim, Chang~Min Park, and Jong~Chul Ye.
        \newblock Self-evolving vision transformer for chest x-ray diagnosis through knowledge distillation.
        \newblock \emph{Nature communications}, 13\penalty0 (1):\penalty0 3848, 2022.
        
        \bibitem[Azizi et~al.(2021)Azizi, Mustafa, Ryan, Beaver, Freyberg, Deaton, Loh, Karthikesalingam, Kornblith, Chen, et~al.]{azizi2021big}
        Shekoofeh Azizi, Basil Mustafa, Fiona Ryan, Zachary Beaver, Jan Freyberg, Jonathan Deaton, Aaron Loh, Alan Karthikesalingam, Simon Kornblith, Ting Chen, et~al.
        \newblock Big self-supervised models advance medical image classification.
        \newblock In \emph{Proceedings of the IEEE/CVF international conference on computer vision}, pages 3478--3488, 2021.
        
        \bibitem[Azizi et~al.(2023)Azizi, Culp, Freyberg, Mustafa, Baur, Kornblith, Chen, Tomasev, Mitrovi{\'c}, Strachan, et~al.]{azizi2023robust}
        Shekoofeh Azizi, Laura Culp, Jan Freyberg, Basil Mustafa, Sebastien Baur, Simon Kornblith, Ting Chen, Nenad Tomasev, Jovana Mitrovi{\'c}, Patricia Strachan, et~al.
        \newblock Robust and data-efficient generalization of self-supervised machine learning for diagnostic imaging.
        \newblock \emph{Nature Biomedical Engineering}, pages 1--24, 2023.
        
        \bibitem[Chen et~al.(2023)Chen, Agarwal, Aggarwal, Safta, Balan, and Brown]{chen2023masked}
        Zekai Chen, Devansh Agarwal, Kshitij Aggarwal, Wiem Safta, Mariann~Micsinai Balan, and Kevin Brown.
        \newblock Masked image modeling advances 3d medical image analysis.
        \newblock In \emph{Proceedings of the IEEE/CVF Winter Conference on Applications of Computer Vision}, pages 1970--1980, 2023.
        
        \bibitem[Xie et~al.(2022)Xie, Zhang, Cao, Lin, Bao, Yao, Dai, and Hu]{xie2022simmim}
        Zhenda Xie, Zheng Zhang, Yue Cao, Yutong Lin, Jianmin Bao, Zhuliang Yao, Qi~Dai, and Han Hu.
        \newblock Simmim: A simple framework for masked image modeling.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 9653--9663, 2022.
        
        \bibitem[Hosseinzadeh~Taher et~al.(2023)Hosseinzadeh~Taher, Gotway, and Liang]{hosseinzadeh2023towards}
        Mohammad~Reza Hosseinzadeh~Taher, Michael~B Gotway, and Jianming Liang.
        \newblock Towards foundation models learned from anatomy in medical imaging via self-supervision.
        \newblock In \emph{MICCAI Workshop on Domain Adaptation and Representation Transfer}, pages 94--104. Springer, 2023.
        
        \bibitem[Filiot et~al.(2023)Filiot, Ghermi, Olivier, Jacob, Fidon, Mac~Kain, Saillard, and Schiratti]{filiot2023scaling}
        Alexandre Filiot, Ridouane Ghermi, Antoine Olivier, Paul Jacob, Lucas Fidon, Alice Mac~Kain, Charlie Saillard, and Jean-Baptiste Schiratti.
        \newblock Scaling self-supervised learning for histopathology with masked image modeling.
        \newblock \emph{medRxiv}, pages 2023--07, 2023.
        \newblock URL \url{https://www.medrxiv.org/content/10.1101/2023.07.21.23292757v2.full.pdf}.
        
        \bibitem[Vorontsov et~al.(2023)Vorontsov, Bozkurt, Casson, Shaikovski, Zelechowski, Liu, Mathieu, van Eck, Lee, Viret, Robert, Wang, Kunz, Lee, Bernhard, Godrich, Oakley, Millar, Hanna, Retamero, Moye, Yousfi, Kanan, Klimstra, Rothrock, and Fuchs]{vorontsov2023virchow}
        Eugene Vorontsov, Alican Bozkurt, Adam Casson, George Shaikovski, Michal Zelechowski, Siqi Liu, Philippe Mathieu, Alexander van Eck, Donghun Lee, Julian Viret, Eric Robert, Yi~Kan Wang, Jeremy~D. Kunz, Matthew C.~H. Lee, Jan Bernhard, Ran~A. Godrich, Gerard Oakley, Ewan Millar, Matthew Hanna, Juan Retamero, William~A. Moye, Razik Yousfi, Christopher Kanan, David Klimstra, Brandon Rothrock, and Thomas~J. Fuchs.
        \newblock A foundation model for clinical-grade computational pathology and rare cancers detection.
        \newblock {\em Nature Medicine}, 30:2924--2935, 2024.  
        
        \bibitem[{\c{C}}all{\i} et~al.(2021){\c{C}}all{\i}, Sogancioglu, van Ginneken, van Leeuwen, and Murphy]{ccalli2021deep}
        Erdi {\c{C}}all{\i}, Ecem Sogancioglu, Bram van Ginneken, Kicky~G van Leeuwen, and Keelin Murphy.
        \newblock Deep learning for chest x-ray analysis: A survey.
        \newblock \emph{Medical Image Analysis}, 72:\penalty0 102125, 2021.
        
        \bibitem[Sellergren et~al.(2022)Sellergren, Chen, Nabulsi, Li, Maschinot, Sarna, Huang, Lau, Kalidindi, Etemadi, et~al.]{sellergren2022simplified}
        Andrew~B Sellergren, Christina Chen, Zaid Nabulsi, Yuanzhen Li, Aaron Maschinot, Aaron Sarna, Jenny Huang, Charles Lau, Sreenivasa~Raju Kalidindi, Mozziyar Etemadi, et~al.
        \newblock Simplified transfer learning for chest radiography models using less data.
        \newblock \emph{Radiology}, 305\penalty0 (2):\penalty0 454--465, 2022.
        
        \bibitem[Oakden-Rayner(2020)]{oakden2020exploring}
        Luke Oakden-Rayner.
        \newblock Exploring large-scale public medical image datasets.
        \newblock \emph{Academic radiology}, 27\penalty0 (1):\penalty0 106--112, 2020.
        
        \bibitem[Majkowska et~al.(2020)Majkowska, Mittal, Steiner, Reicher, McKinney, Duggan, Eswaran, Cameron~Chen, Liu, Kalidindi, et~al.]{majkowska2020chest}
        Anna Majkowska, Sid Mittal, David~F Steiner, Joshua~J Reicher, Scott~Mayer McKinney, Gavin~E Duggan, Krish Eswaran, Po-Hsuan Cameron~Chen, Yun Liu, Sreenivasa~Raju Kalidindi, et~al.
        \newblock Chest radiograph interpretation with deep learning models: assessment with radiologist-adjudicated reference standards and population-adjusted evaluation.
        \newblock \emph{Radiology}, 294\penalty0 (2):\penalty0 421--431, 2020.
        
        \bibitem[Gaggion et~al.(2023)Gaggion, Mosquera, Mansilla, Aineseder, Milone, and Ferrante]{gaggion2023chexmask}
        Nicol{\'a}s Gaggion, Candelaria Mosquera, Lucas Mansilla, Martina Aineseder, Diego~H Milone, and Enzo Ferrante.
        \newblock CheXmask: a large-scale dataset of anatomical segmentation masks for multi-center chest x-ray images.  
        \newblock {\em Scientific Data}, 11(1):511, 2024.  
        \newblock Nature Publishing Group UK London. 
        
        \bibitem[Rueckel et~al.(2021)Rueckel, Huemmer, Fieselmann, Ghesu, Mansoor, Schachtner, Wesp, Trappmann, Munawwar, Ricke, et~al.]{rueckel2021pneumothorax}
        Johannes Rueckel, Christian Huemmer, Andreas Fieselmann, Florin-Cristian Ghesu, Awais Mansoor, Balthasar Schachtner, Philipp Wesp, Lena Trappmann, Basel Munawwar, Jens Ricke, et~al.
        \newblock Pneumothorax detection in chest radiographs: optimizing artificial intelligence system for accuracy and confounding bias reduction using in-image annotations in algorithm training.
        \newblock \emph{European radiology}, pages 1--13, 2021.
        
        \bibitem[Endo et~al.(2021)Endo, Krishnan, Krishna, Ng, and Rajpurkar]{endo2021retrieval}
        Mark Endo, Rayan Krishnan, Viswesh Krishna, Andrew~Y Ng, and Pranav Rajpurkar.
        \newblock Retrieval-based chest x-ray report generation using a pre-trained contrastive language-image model.
        \newblock In \emph{Machine Learning for Health}, pages 209--219. PMLR, 2021.
        
        \bibitem[Miura et~al.(2021)Miura, Zhang, Tsai, Langlotz, and Jurafsky]{miura2021improving}
        Yasuhide Miura, Yuhao Zhang, Emily Tsai, Curtis Langlotz, and Dan Jurafsky.
        \newblock Improving factual completeness and consistency of image-to-text radiology report generation.
        \newblock In \emph{Proceedings of the 2021 Conference of the North American Chapter of the Association for Computational Linguistics: Human Language Technologies}, pages 5288--5304, 2021.
        
        \bibitem[Bromley et~al.(1993)Bromley, Guyon, LeCun, S\"{a}ckinger, and Shah]{NIPS1993_288cc0ff}
        Jane Bromley, Isabelle Guyon, Yann LeCun, Eduard S\"{a}ckinger, and Roopak Shah.
        \newblock Signature verification using a "siamese" time delay neural network.
        \newblock In J.~Cowan, G.~Tesauro, and J.~Alspector, editors, \emph{Advances in Neural Information Processing Systems}, volume~6. Morgan-Kaufmann, 1993.
        \newblock URL \url{https://proceedings.neurips.cc/paper_files/paper/1993/file/288cc0ff022877bd3df94bc9360b9c5d-Paper.pdf}.
        
        \bibitem[Tarvainen and Valpola(2017)]{tarvainen2017mean}
        Antti Tarvainen and Harri Valpola.
        \newblock Mean teachers are better role models: Weight-averaged consistency targets improve semi-supervised deep learning results.
        \newblock \emph{Advances in neural information processing systems}, 30, 2017.
        
        \bibitem[Wang et~al.(2022{\natexlab{c}})Wang, Fan, Tian, Kihara, and Chen]{wang2022importance}
        Xiao Wang, Haoqi Fan, Yuandong Tian, Daisuke Kihara, and Xinlei Chen.
        \newblock On the importance of asymmetry for siamese representation learning.
        \newblock In \emph{Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition}, pages 16570--16579, 2022{\natexlab{c}}.
        
        \bibitem[Sablayrolles et~al.(2018)Sablayrolles, Douze, Schmid, and J{\'e}gou]{sablayrolles2018spreading}
        Alexandre Sablayrolles, Matthijs Douze, Cordelia Schmid, and Herv{\'e} J{\'e}gou.
        \newblock Spreading vectors for similarity search.
        \newblock In \emph{International Conference on Learning Representations}, 2018.
        
        \bibitem[Bardes et~al.(2022)Bardes, Ponce, and LeCun]{bardes2022vicregl}
        Adrien Bardes, Jean Ponce, and Yann LeCun.
        \newblock Vicregl: Self-supervised learning of local visual features.
        \newblock \emph{Advances in Neural Information Processing Systems}, 35:\penalty0 8799--8810, 2022.
        
        \bibitem[Haque et~al.(2023)Haque, Dubey, Danciu, Justice, Ovchinnikova, and Hinkle]{haque2023effect}
        Md~Inzamam~Ul Haque, Abhishek~K Dubey, Ioana Danciu, Amy~C Justice, Olga~S Ovchinnikova, and Jacob~D Hinkle.
        \newblock Effect of image resolution on automated classification of chest x-rays.
        \newblock \emph{Journal of Medical Imaging}, 10\penalty0 (4):\penalty0 044503--044503, 2023.
        
        \bibitem[Sabottke and Spieler(2020)]{sabottke2020effect}
        Carl~F Sabottke and Bradley~M Spieler.
        \newblock The effect of image resolution on deep learning in radiography.
        \newblock \emph{Radiology: Artificial Intelligence}, 2\penalty0 (1):\penalty0 e190015, 2020.
        
        \bibitem[Tanno et~al.(2023)Tanno, Barrett, Sellergren, Ghaisas, Dathathri, See, Welbl, Singhal, Azizi, Tu, et~al.]{tanno2023consensus}
        Ryutaro Tanno, David~GT Barrett, Andrew Sellergren, Sumedh Ghaisas, Sumanth Dathathri, Abigail See, Johannes Welbl, Karan Singhal, Shekoofeh Azizi, Tao Tu, et~al.
        \newblock Consensus, dissensus and synergy between clinicians and specialist foundation models in radiology report generation.
        \newblock \emph{arXiv preprint arXiv:2311.18260}, 2023.
        \newblock URL \url{https://arxiv.org/pdf/2311.18260.pdf}.
        
        \bibitem[Duffy et~al.(2022)Duffy, Clarke, Christensen, He, Yuan, Cheng, and Ouyang]{duffy_confounders_2022}
        Grant Duffy, Shoa~L. Clarke, Matthew Christensen, Bryan He, Neal Yuan, Susan Cheng, and David Ouyang.
        \newblock Confounders mediate {AI} prediction of demographics in medical imaging.
        \newblock \emph{npj Digital Medicine}, 5\penalty0 (1):\penalty0 188, 2022.
        \newblock ISSN 2398-6352.
        \newblock \doi{10.1038/s41746-022-00720-8}.
        \newblock URL \url{https://www.nature.com/articles/s41746-022-00720-8}.
        
        \bibitem[Pedregosa et~al.(2011)Pedregosa, Varoquaux, Gramfort, Michel, Thirion, Grisel, Blondel, Prettenhofer, Weiss, Dubourg, Vanderplas, Passos, Cournapeau, Brucher, Perrot, and Duchesnay]{scikitlearn}
        F.~Pedregosa, G.~Varoquaux, A.~Gramfort, V.~Michel, B.~Thirion, O.~Grisel, M.~Blondel, P.~Prettenhofer, R.~Weiss, V.~Dubourg, J.~Vanderplas, A.~Passos, D.~Cournapeau, M.~Brucher, M.~Perrot, and E.~Duchesnay.
        \newblock Scikit-learn: Machine learning in {P}ython.
        \newblock \emph{Journal of Machine Learning Research}, 12:\penalty0 2825--2830, 2011.

        % \bibitem[Jiang et~al.(2024)Jiang, Dongsheng, Liu, Yuchen, Liu, Songlin, Zhao, Jin'e, Zhang, Hao, Gao, Zhen, Zhang, Xiaopeng, Li, Jin, Xiong, Hongkai]{jiang_clip_2024}
        % Dongsheng Jiang, Yuchen Liu, Liu Songlin, Jin'e Zhao, Hao Zhang, Zhen Gao, Xiaopeng Zhang, Jin Li, and Hongkai Xiong.
        % \newblock \emph{arXiv preprint arXiv:2310.08825}, 2024.
        % \newblock URL \url{https://arxiv.org/pdf/2310.08825.pdf}
        
    \end{thebibliography}

==> experiment_and_code/aml_runs.tex <==
%%%%%%%%%%%%%%%%%%%% Ablation %%%%%%%%%%%%%%%%%%%%
%# 518px - "plucky_wheel_sspghcjfd9"
%# 448px - "affable_malanga_y3g3htkl0t"
%# 336px - "bold_soca_85lf992vt1"
%# 224px - "clever_animal_n9zpw415jx"
%# No-pretrain-weights - "jolly_glass_p4nf327dhl"
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%% Ablation %%%%%%%%%%%%%%%%%%%%
% Training dataset size vs VinDr performance (Candid-PTX Validation)

%vitb-197k-mimic pre-train: "joyful_shirt_fbs7fpkptl"
%"raddio_biovil_subset_of_mimic_step30k": "ashy_plane_fysjy7yyjt",

%vitb-355k-mimic-nih-e100: "keen_sugar_hkgyyf18gr" 40k
%"vitb-355k-mimic-nih-e100-40k": "loyal_dog_l68jvr2rkw",

% "vitb-657k-padchest-chxpert-mimic-nih-e100" "salmon_cushion_909pc1x8b0"
%"vitb-657k-s60k": "quirky_tent_9psz2jyp6z",

% ViT-B Baseline 880k - "nifty_garden_l55z0p99qz"
%"raddino-ep100-s60k-new-baseline-60k": "teal_camel_zsrzx2rcx0",
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



%%%%%%%%%%%%%%%%%%%%%%Ablation%%%%%%%%%%%%%%%%%%%%
% vitg-hub-5-seed -- hungry_soca_xt2gnjy2ls



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% Image Classification VinDR
% "mrm-baseline-5seed": "olden_ant_4p8f3g4h9m"

% Image Classification Candid-PTX
% "mrm_candid_5seed": "HD_d1a2c18a-0d41-46ed-bdeb-89a24e332edc",

% Image Classification RSNA Pneumonia
%mrm_baseline_pneumonia_5_seeds: HD_cedb37ad-b9b6-4791-b9b1-5c152d7d752a

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


%%%%%%%%%%%%%%%%%%%%%% Text Generation %%%%%%%%%%%%%%%%%%%%
% Control - RadDINO (biovil subset) final         dino_run_id, dino_step_id = "lemon_star_f752p5wmgg", 45000

% Rad-DINO (full)
% https://ml.azure.com/experiments/id/59aaa49c-33dc-40fd-b1df-b19837753927/runs/nifty_garden_l55z0p99qz?wsid=/subscriptions/a85ceddd-892e-4637-ae4b-67d15ddf5f2b/resourceGroups/RadiomicsNN/providers/Microsoft.MachineLearningServices/workspaces/BiomedImagingWestUS2&tid=72f988bf-86f1-41af-91ab-2d7cd011db47
%dino_run_id = "nifty_garden_l55z0p99qz"
%dino_step_id = 60000



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> experiment_and_code/notes_from_teo.tex <==
% Discussion with Teo-Ozan
% AE -- Rather chronic or incidental finding (e.g., aortic enlargement) - PA (mediastinum can be better assessed).
% PL-T -- Rather chronic.
% PF -> develops over years, chronic. (less common in ICU, you need out-patient context, you will not have this as an indication)
% TB (infection, out-patient, incidental finding, less frequent -- specific ward, isolated) 

% You could do spine x-ray to assess spine (vertebral changes) - To describe incidental finding by checking the lateral scan.

% Value of lateral over frontal - To see hidden lesions (behind the diaphram, heart, mediastinum) 

% Costrophenic-angle (posterior-side) -> laterals can help to see posterior angle of it, to detect pleural effusion. Look for the keyword "lateral" - if it's an exception case.

% Ostopenia -> More global! 


==> experiment_and_code/reports_analysis.tex <==
%Basic Analysis on MIMIC-CXR Reports (Findings Section)
%"pleural effusion" was found in 150k studies
%"cardiomegaly" over 50k studies
%"opacity" was found in 30299 studies
%"fibrosis" was found in 1116 studies 
%"tuberculosis" was found in 317 studies
%Out of 227.8k reports

==> experiment_and_code/temporary.tex <==
\section{Temporary table to monitor segmentation results}

\begin{table}[t]
    \scriptsize % temporarily
    \centering
    \caption{Temporary. * means new checkpoint.}
    \vspace{0.5cm}
    \begin{tabular}{
        l
        c
        c
        c
        S[table-format=2.1 (2), separate-uncertainty=true]
        S[table-format=2.1 (2), separate-uncertainty=true]
        S[table-format=2.1 (2), separate-uncertainty=true]
        S[table-format=2.1 (2), separate-uncertainty=true]
        S[table-format=2.1 (2), separate-uncertainty=true]
        S[table-format=2.1 (2), separate-uncertainty=true]
    }
        \toprule
        \textbf{Model} & \textbf{Type} & \textbf{\# intermediate} & \textbf{Frozen backbone} & {\textbf{Lungs}} & {\textbf{Lung zones}} & {\textbf{Pneumothorax}} \cite{feng2021curation} & {\textbf{Chest tubes}} & {\textbf{Ribs}} \cite{nguyen2021vindrribcxr} \\
        \midrule
        U-Net*              & ---     & --- & No  & 98.6 \pm 0.9 & 95.6 \pm 3.8 & 83.9 \pm 22.3 & 58.6 \pm 19.1 & 89.2 \pm 2.7 \\
        U-Net (224) & ---  & --- & No & 98.3 (1.2) & 95.5 (3.8) & 78.3 (32.7) & 41.4 (26.1) & 84.8 (3.7) \\
        \midrule
        \biovil             & Interp. & 1   & Yes & 83.4 \pm 4.7 & 71.2 \pm 6.2 & 28.5 \pm 57.0 & 4.0 \pm 11.1 & 59.5 \pm 7.1 \\
        % Model               Type    Layers Frozen  Lungs          Zones          PTX             Tubes          Ribs
        \biomedclip          & Interp. & 1   & Yes & 90.9 \pm 3.3 & 78.5 \pm 6.5 & 29.0 \pm 37.8 & 1.9 \pm 10.6 & 67.6 \pm 6.2 \\
        % Model               Type    Layers Frozen  Lungs          Zones          PTX             Tubes          Ribs
        \raddinoViTB (no MIM) & Interp. & 1   & Yes & 91.7 \pm 3.2 & 81.1 \pm 7.8 & 37.1 \pm 45.7 & 24.5 \pm 15.0 & 67.3 \pm 5.3 \\
        % Model               Type    Layers Frozen  Lungs          Zones          PTX             Tubes          Ribs
        \raddinoViTB          & Interp. & 1   & Yes & 96.2 \pm 1.5 & 87.9 \pm 5.4 & 60.8 \pm 38.4 & 32.1 \pm 10.0 & 73.2 \pm 5.5 \\
        \raddinoViTB*        & Interp. & 1   & Yes & 95.9 \pm 1.6 & 87.8 \pm 5.5 & 60.3 \pm 40.1 & 26.8 \pm 8.2 & 73.3 \pm 4.7 \\
        
        \raddinoViTB           & Interp. & 4 & Yes & 97.1 (1.4) & 90.0 (4.4) & 64.7 (35.2) & 32.3 (10.6) & 76.3 (4.3) \\
        
        \addlinespace
        
        \raddinoViTB & Interp. & 1 & No & 95.7 (1.4) & 93.1 (3.2) & 69.6 (61.3) & 37.8 (11.1) & 83.2 (3.2) \\
        \raddinoViTB & Interp. & 4 & No & 96.9 (1.2)  & 94.9 (3.4) & 73.5 (42.6) & 44.2 (12.3) & 84.0 (3.7) \\

        \addlinespace
        
        % \raddinoViTB     & ViTDet (old) & 4   & Yes & 98.2 \pm 1.3 & 93.4 \pm 4.5 & 69.5 \pm 36.6 & 42.1 \pm 16.4 & 84.5 \pm 3.7 \\  % batch norm, fix mean & std
        \raddinoViTB          & ViTDet  & 4   & Yes & 98.3 \pm 1.2             & 93.5 \pm 3.9 & 73.8 \pm 31.9 & 47.4 \pm 17.8 & 86.6 \pm 3.5 \\  % all extras
        \raddinoViTB*          & ViTDet  & 4   & Yes & 98.4 \pm 1.2 & 93.8 \pm 4.2 & 72.8 \pm 29.8 & 46.1 \pm 17.8 & 87.7 \pm 3.4 \\  % new checkpoint
        \raddinoViTB (1022)         & ViTDet  & 4   & Yes & 98.3 \pm 1.2             & 93.6 \pm 4.0 & 75.4 \pm 26.6 & 46.1 \pm 18.7 & 86.4 \pm 3.5 \\  % inference? at 1022 resolution
        \bottomrule
    \end{tabular}
    \label{tab:segmentation_benchmarks_si}
\end{table}
